New trends in indoor positioning based on WiFi and machine learning: A systematic review

Currently there is no standard indoor positioning system, similar to outdoor GPS. However, WiFi signals have been used in a large number of proposals to achieve the above positioning, many of which use machine learning to do so. But what are the most commonly used techniques in machine learning? What accuracy do they achieve? Where have they been tested? This article presents a systematic review of works between 2019 and 2021 that use WiFi as the signal for positioning and machine learning models to estimate indoor position. 64 papers have been identified as relevant, which have been systematically analyzed for a better understanding of the current situation in different aspects. The results show that indoor positioning based on WiFi trends use neural network-based models, evaluated in empirical experiments. Despite this, many works still conduct an assessment in small areas, which can influence the goodness of the results presented.

==> Tables/contents4.tex <==
\cite{Jang2018753}&	2018&	wifi&	sim&	$520$&	$19937$&	UJIIndoorLoc&	Y&	CNN&	&	&	95.76\% floor level&	RSSI	\\\midrule
\cite{Gomes2018537}&	2018&	wifi&	sim&	$N/A$&	$N/A$&	UCI ML Repository&	Y&	RF&	&	&	98.3\% floor level&	RSSI	\\\midrule
\cite{Chen2018}&	2018&	wifi&	exp&	$20$&	$2100$&	\SI{8250}{\square\meter}&	Y&	DNN&	&	\SI{3,95}{\meter}&	std = 2.72 &	RSSI	\\\midrule
\cite{RN8783}&	2018&	wifi&	exp&	$16$&	$202$&	\SI{806}{\square\meter}&	Y&	SMN&	PCA&	\SI{1,847}{\meter}&	std = 1.04&	RSSI	\\\midrule
\cite{RN8593}&	2018&	wifi&	sim&	$520$&	$19937$&	UJIIndoorLoc&	Y&	DQN&	&	&	78.79\% in \SI{1}{\meter}&	RSSI	\\\midrule
\cite{RN8568}&	2018&	wifi&	exp&	$50$&	$180$&	\SI{75}{\square\meter}&	Y&	RFR&	&	\SI{1,29}{\meter}&	90\% in \SI{3}{\meter}&	RSSI	\\\midrule
\cite{RN8511}&	2018&	wifi&	exp&	$N/A$&	$N/A$&	NULL&	Y&	DNN&	&	&	83.6\% floor with people , 99.6\% without&	RSSI	\\\midrule
\multirow{2}[2]{*}{\cite{RN8526}}&	\multirow{2}[2]{*}{2018}&	wifi&	sim&	$N/A$&	$N/A$&	UJI Library &	Y&	RNN&	&	\SI{2,482}{\meter}&	99.6\% floor level&	RSSI	\\\cmidrule(lr){3-12}
&	&	wifi&	sim&	$N/A$&	$N/A$&	UJI Library &	Y&	LSTM&	&	\SI{2,599}{\meter}&	99.5\% floor level&	RSSI	\\\midrule
\cite{RN8612}&	2018&	wifi&	sim&	$520$&	$19937$&	UJIIndoorLoc&	Y&	RDF&	&	\SI{6,72}{\meter}&	std = 4.82&	RSSI	\\\midrule
\cite{RN8648}&	2018&	wifi&	exp&	$7$&	$101$&	\SI{404,5}{\square\meter}&	Y&	FF-DNN&	&	&	RMSE = \SI{0,32}{\meter} , 53.123\% in \SI{0,5}{\meter}&	RSSI	\\\midrule
\cite{RN8445}&	2018&	wifi&	exp&	$4$&	$25$&	\SI{80}{\square\meter}&	N&	RF&	&	\SI{0,4033}{\meter}&	&	CSI	\\\midrule
\cite{RN8622}&	2018&	wifi&	exp&	$4$&	$67$&	\SI{1664}{\square\meter}&	Y&	SVM&	&	\SI{1,34}{\meter}&	&	RSSI	\\\midrule
\cite{RN8667}&	2018&	wifi&	sim&	$520$&	$19937$&	UJIIndoorLoc&	Y&	CNN&	&	\SI{2,77}{\meter}&	100\% for floor prediction&	RSSI	\\\midrule
\cite{RN8498}&	2018&	wifi&	exp&	$N/A$&	$N/A$&	NULL&	NULL&	SVR&	RBF Kernel&	&	95\% in \SI{1,81}{\meter}&	RSSI	\\\midrule
\cite{RN8629}&	2018&	wifi&	exp&	$40$&	$180$&	\SI{1209}{\square\meter}&	Y&	RF&	&	&	95\% accuracy 1.5x\SI{1,5}{\meter}&	RSSI	\\\midrule
\cite{RN8482}&	2018&	wifi&	exp&	$8$&	$40$&	\SI{580}{\square\meter}&	Y&	RVFL&	&	\SI{0,43}{\meter}&	RMSE = \SI{58,30}{\meter}&	RSSI	\\\midrule
\multirow{2}[2]{*}{\cite{RN8508}}&	\multirow{2}[2]{*}{2018}&	wifi&	sim&	$4$&	$36$&	\SI{441}{\square\meter}&	N&	RVM&	PLS&	\SI{0,84}{\meter}&	&	RSSI	\\\cmidrule(lr){3-12}
&	&	wifi&	exp&	$6$&	$25$&	\SI{156}{\square\meter}&	Y&	RVM&	PLS&	&	41\% in \SI{1}{\meter} and 91\% in \SI{2}{\meter}&	RSSI	\\\midrule
\cite{Belay20171763}&	2017&	wifi&	exp&	$3$&	$110$&	\SI{109,25}{\square\meter}&	N&	FF-DNN&	&	&	RMSE = \SI{0,6782}{\meter}&	RSSI	\\\midrule
\multirow{2}[2]{*}{\cite{Amirisoori20174144}}&	\multirow{2}[2]{*}{2017}&	wifi&	exp&	$4$&	$N/A$&	NULL&	N&	ANN&	&	&	RMSE = \SI{1,1045}{\meter}&	RSSI	\\\cmidrule(lr){3-12}
&	&	wifi&	exp&	$6$&	$N/A$&	NULL&	N&	ANN&	&	&	RMSE = \SI{1,2288}{\meter}&	RSSI	\\\midrule
\cite{RN8684}&	2017&	wifi&	exp&	$16$&	$126$&	\SI{304}{\square\meter}&	Y&	SVM&	&	\SI{1,43}{\meter}&	&	RSSI	\\\midrule
\cite{RN8779}&	2017&	wifi&	sim&	$6$&	$441$&	\SI{100}{\square\meter}&	N&	LS-SVM&	&	\SI{2,56}{\meter}&	&	RSSI	\\\midrule
\cite{RN8758}&	2017&	wifi&	exp&	$38$&	$411$&	\SI{600}{\square\meter}&	Y&	ELM&	&	\SI{1,91}{\meter}&	&	RSSI	\\\midrule
\cite{RN8866}&	2017&	wifi&	exp&	$28$&	$67$&	\SI{30}{\square\meter}&	N&	ANN&	&	\SI{2,2}{\meter}&	&	RSSI	\\\midrule
\cite{RN8825}&	2017&	wifi&	exp&	$185$&	$480$&	NULL&	Y&	SVM&	&	&	100\% shop level&	RSSI	\\\midrule
\cite{RN8838}&	2017&	wifi&	sim&	$520$&	$19937$&	UJIIndoorLoc&	Y&	DNN&	&	&	92\% floor recognition&	RSSI	\\\midrule
\cite{RN8745}&	2017&	wifi&	exp&	$8$&	$48$&	\SI{53,35}{\square\meter}&	N&	RVR&	&	&	86.2\% in \SI{1,5}{\meter} and 90.4\% in \SI{2}{\meter}&	RSSI	\\\midrule
\cite{RN8773}&	2017&	wifi&	exp&	$N/A$&	$N/A$&	NULL&	Y&	SVM&	&	&	97.31\% flat and 88.38\% floor&	RSSI	\\\midrule
\cite{Abdullah2016362}&	2016&	wifi&	exp&	$22$&	$84$&	\SI{387,75}{\square\meter}&	Y&	BPNN&	&	\SI{0,98}{\meter}&	&	RSSI	\\\midrule
\cite{RN8889}&	2016&	wifi&	sim&	$4$&	$25$&	\SI{400}{\square\meter}&	N&	MLP-ANN&	&	\SI{0,27}{\meter}&	std = 0.36&	RSSI	\\\midrule
\cite{RN9065}&	2016&	wifi&	sim&	$N/A$&	$N/A$&	NULL&	NULL&	EB-ANN&	&	&	RMSE = \SI{0,4991}{\meter}&	RSSI	\\\midrule
\cite{RN9074}&	2016&	wifi&	exp&	$5$&	$54$&	\SI{150}{\square\meter}&	Y&	SVR&	&	&	70\% in \SI{5}{\meter}&	RSSI	\\\midrule
\cite{RN9005}&	2016&	wifi&	exp&	$16$&	$188$&	\SI{1125}{\square\meter}&	Y&	ANN&	&	\SI{1,893}{\meter}&	90\% in \SI{2,971}{\meter}&	RSSI	\\\midrule
\multirow{2}[2]{*}{\cite{RN8908}}&	\multirow{2}[2]{*}{2016}&	wifi&	sim&	$12$&	$1600$&	\SI{1600}{\square\meter}&	N&	SVR&	&	&	RMSE = \SI{1,42}{\meter}&	RSSI	\\\cmidrule(lr){3-12}
&	&	wifi&	exp&	$13$&	$116$&	\SI{1000}{\square\meter}&	Y&	SVR&	&	&	RMSE = \SI{1,8}{\meter} , 74\% in \SI{2}{\meter}&	RSSI	\\\midrule
\multirow{2}[2]{*}{\cite{RN8877}}&	\multirow{2}[2]{*}{2016}&	wifi&	exp&	$N/A$&	$112$&	\SI{460}{\square\meter}&	Y&	SVM&	&	\SI{1,2}{\meter}&	&	RSSI	\\\cmidrule(lr){3-12}
&	&	wifi&	exp&	$N/A$&	$112$&	\SI{460}{\square\meter}&	Y&	SVM&	&	\SI{2,1}{\meter}&	&	RSSI	\\\midrule
